A proof using B\"ohme's Lemma that no Petersen family graph has a flat embedding

Sachs and Conway-Gordon used linking number and a beautiful counting argument to prove that every graph in the Petersen family is intrinsically linked (have a pair of disjoint cycles that form a nonsplit link in every spatial embedding) and thus each family member has no flat spatial embedding (an embedding for which every cycle bounds a disk with interior disjoint from the graph). We give an alternate proof that every Petersen family graph has no flat embedding by applying B\"{o}hme's Lemma and the Jordan-Brouwer Separation Theorem.

==> OldVersion.tex <==
%\documentclass{article}
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{caption}
\usepackage{subcaption}

\title{A proof that the Petersen Family graphs are not flat, using B\"ohme's Lemma}
\author{Joel Foisy, Catherine Jacobs, Trinity Paquin, Morgan Schalizki, Henry Stringer}
\date{November 2022}



\begin{document}
\maketitle

\begin{abstract}

Sachs and Conway-Gordon (for $K_6$) showed that each Petersen family graphs has no linkless spatial embedding and thus no flat spatial embedding. We demonstrate an alternate proof that each Petersen family graph has no flat spatial embedding, using B\"{o}hme's Lemma and the Jordan-Brouwer Separation Theorem.
\end{abstract}
\section{Introduction}

%In this paper we will be exploring a new proof of how the Petersen Family Graphs such as $K_6$ and $P_7$ are not flat.

\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=.525\linewidth]{k_6.png}
        \captionof{figure}{$K_6$}
        \label{fig:test1}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=.4\linewidth]{p7.jpg}
        \captionof{figure}{$P_7$}
        \label{fig:test2}
    \end{subfigure}
\end{figure*}

The \textit{Petersen Family} of graphs includes $K_6$ and the six other graphs obtained from $K_6$ by $\Delta-Y$ and $Y-\Delta$ exchanges. The family includes the classic Petersen Graph. Conway-Gordon \cite{cg} and Sachs \cite{sachs} proved that $K_6$ is intrinsically linked (has a pair of nonsplit linked cycles in every spatial embedding), and Sachs further proved that every graph in the Petersen Family Graphs is intrinsic linked. As a consequence of being intrinsically linked, every graph in the Petersen Family is has no flat embedding (a spatial embedding is \textit{flat} if every cycle bounds a disk with interior disjoint from the embedded graph, that is, every cycle can be paneled).

We have devised a new family of proofs that the Petersen Family graphs have no flat embedding. To do so, we use B\"{o}hme's Lemma which states that for a flatly embedded graph and a set of cycles that have pair-wise intersection either connected or empty, then all cycles in the set can be simultaneously paneled with disks that have interiors disjoint from the graph and from each other. We call a set of cycles that satisfies the hypotheses of B\"{o}hme's Lemma a \textit{B\"{o}hme system}. We will also use the Jordan-Brouwer Separation Theorem which implies that any sphere formed by a B\"{o}hme system forms an inside and an outside region, when its complement is taken in ${\mathbb R}^3$. 

For each Petersen Family graph, we suppose it has a flat embedding. We then find a B\"ohme system such that some sphere formed by paneling it via B\"ohme's Lemma must be punctured by an edge. This leads to a contradictions for each Petersen family graph having a flat embedding. 

%As we move between the graphs in the Petersen family graphs, we perform $\Delta$-Y and Y-$\Delta$ exchanges. This encouraged the idea to look at the affects $\Delta$-Y and Y-$\Delta$ exchanges have on spherical flatness. As a result we were able to prove via contrapositive that $\Delta$-Y exchanges preserve spherical flatness.

\section{Background}

A \emph{spatial embedding} of a graph is a way to place a graph in space, so that vertices are points and edges are arcs that meet only at vertices. All embeddings considered are tame (in the PL category). 

Suppose we have a three cycle with vertices $a,b,c$. To perform a $\Delta$ -Y exchange, an extra vertex $y$ is added, edges $(a,b),(b,c),$and$(c,a)$ are removed, and the edges $(a,y),(b,y),$ and $(c,y)$ are added. To perform a Y-$\Delta$ exchange, we begin with the Y shape, having vertices $a,b,c, y$ and edges $(a,y),(b,y),$ and $(c,y)$. We remove the $y$ vertex and all edges including $y$ and then add edges $(a,b),(b,c),$and$(c,a)$ to make our triangle.
%Note that for $Y_\Delta$ exchanges any spatially embedded $G$ can be stretched or adjusted and the edges of $\Delta$ can be placed in ways which do not intersect the rest of the graph and so that every 2-path in the $Y$ is ambient isotopic to an edge of $\Delta$.

%\begin{center}
%\includegraphics[scale=.5]{Triangle-Y.png}
%\end{center}
 
We know that both $\Delta$-Y (Motwani, Ragunathan, Saran) and Y-$\Delta$ (Robertson, Seymour, and Thomas) exchanges preserve intrinsic linking. Also, it has been shown that Y-$\Delta$ preserves planarity but $\Delta$-Y does not always.
\noindent

{\bf Spherically flat graphs.} First, a spatial graph $f(G)$ is \emph{flat} if it is possible to attach a topological disk to every cycle, $C$, of $G$ so that the disk intersects $C$ along its boundary, and the interior of the disk is disjoint from $f(G)$. Every flat embedding is linkless. Robertson, Seymour and Thomas showed that a graph has a flat embedding if and only if it  has a linkless embedding. We'll call a graph $G$ \emph{flat} if it has a flat spatial embedding (Robertson, Seymour, and Thomas).\\

A graph $G$ is \emph{spherically flat} if there is a flat spatial embedding of $G$, $f(G)$, such that every planar subgraph $P$ of $G$ lies on an embedded sphere $S$ that intersects $f(G)$ only in $f(P)$. By the Jordan-Brouwer theorem, any vertex or edge in $f(G)-f(P)$ lies on one side of $S$ (for an edge, its endpoints lies in $S$).\\

Note that if $G$ is spherically flat, then $G$ is flat (every cycle is itself a planar subgraph, so lies on a sphere, and from there, take a bounding disk) and $G$ has a linkless embedding.\\

\section{Petersen family graphs not flat}
\begin{itemize}


\item $K_6$

\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=.525\linewidth]{k_6.png}
        \captionof{figure}{$K_6$}
        \label{fig:test1}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=.4\linewidth]{k6extra.png}
        \captionof{figure}{Spatial embedding of $K_6$}
        \label{fig:test2}
    \end{subfigure}
\end{figure*}
%\ref{test}

By way of contradiction suppose that $G = K_6$ has a flat embedding. Consider the cycles:
\begin{center}
    $C_1 = \{(bef), (bce), (cef), (bcf)\}$,\\
    $C_2 = \{(bef), (abe), (aef), (abf)\}$,\\
    $C_3 = \{(bef), (bde), (def), (bdf)\}$.\\
\end{center}
Let $C = \cup^3_{i=1}C_i$. Note that the cycles above are induced cycles where $C_1 \subset G[cbef], C_2 \subset G[abef]$, and $C_3 \subset G[dbef]$ and notice they all have the cycle $(b e f) \subset C_i$ for $i = 1, 2, 3$. As all the cycles of C all have connected pairwise intersections and $K_6$ has a flat embedding, we can apply B\"{o}hme's Lemma to get disks $D_1, ..., D_{12}$. Let $T_i = C_i \cup (\cup^{k}_j D_j)$ where $i = 1, 2, 3$, $j = 4i - 3$ and $k = j + 4$. As we panel $C_1$, we form a sphere $T_1$, then by Jordan-Brouwer Theorem applied to $T_1$, we then get an inside and outside ball, $B_1$ and $B_2$ respectively. Without loss of generality as $\overline{ad} \not\in T_1$, we may assume that $\overline{ad} \in B_1$. As $\overline{ad} \in B_1$ and $a \in T_2, d \in T_3$ then $T_2, T_3 \subset B_1 \cup T_1$. This means that $T_2$ and $T_3$ are in the closure of the inside ball of $T_1$. Now similarly form an inside and outside ball for $T_2$. Without loss of generality suppose that $T_3$ is in the closure of the inner ball of $T_2$. As $d \not\in T_2$ and $d \in T_3$, d is in the inner ball of $T_2$. As $T_2$ is inside $T_1$ and $c \in T_1$, c is outside $T_2$. As there exists an edge between d and c and c and d are on opposite sides of $T_2$, we have an edge passing through a disk of $T_2$.  This brings us a contradiction. 

\item $K_{3,3,1}$
\begin{center}
    \includegraphics{K_3,3,1.png}
\end{center}

Assume by way of contradiction that $K_{3,3,1}$ is flat. Thus there is a spatial embedding such that, for every cycle, there is a disk bounded by the cycles with an interior disjoint from the rest of the graph. Consider the collection of cycles:
\begin{itemize}
    \item $\mathcal{S}_1 = \{(a2c3),(a1c2),(a1c3)\} \subseteq G[ac123]$ 
    \item $\mathcal{S}_2 = \{(a2c3),(3b2c),(3b2a)\} \subseteq G[abc123]$ 
    \item $\mathcal{S}_3 = \{(a2c3),(c2v),(cv3),(3va), (av2)\} \subseteq G[acv23]$ 
\end{itemize}
Notice the subgraphs above are induced subgraphs of $K_{3,3,1}$ and each form a B\"ohme sphere. Panel each cycle to form the B\"ohme sphere. These B\"ohme spheres are comprised of three and four cycles and they all share the same base cycle $(a2c3)$. Since 1 and b are connected, by the Jordan-Brouwer theorem, they must both be inside or both be outside of the sphere generated by $\mathcal{S}_1$. Without loss of generality assume they are both outside of the sphere generated by $\mathcal{S}_1$. Then since b is outside of the sphere generated by $\mathcal{S}_1$, the sphere generated by $\mathcal{S}_2$ must lie in the closure of the region outside of the sphere generated by $\mathcal{S}_1$. Furthermore, since v and b are connected, by the Jordan-Brouwer Theorem, they must both be inside or both be outside of the sphere generated by $\mathcal{S}_2$. Without loss of generality assume they are both outside of the sphere generated by $\mathcal{S}_2$. Then since v is outside of the sphere generated by $\mathcal{S}_2$, the sphere generated by $\mathcal{S}_3$ must lie in the closure of the region outside of the sphere generated by $\mathcal{S}_3$. However, consider the edge between v and 1. V is outside of the sphere generated by $\mathcal{S}_2$, however, 1 is inside the sphere generated by $\mathcal{S}_2$. However, since they are connected they both must lie inside or outside the sphere generated by $\mathcal{S}_2$ by the Jordan-Brouwer theorem. Thus we have a contradiction and $K_{3,3,1}$ is not flat and thus not spherically flat.

\item $K_{4,4} - e$ where $e= \overline{4a}$

\begin{center}
 \includegraphics{k44-4a.jpg}
    \includegraphics{k44-e.jpg}
\end{center}

Assume by way of contradiction that $K_{4,4} - e$ is flat. Then by definition of flat, there is a spacial embedding, such that for each cycle there is a disk bounded by the cycle with an interior disjoint from the rest of the graph. Consider the spheres ($S_i$ where $i \in \{1,2,3\}$) formed by panelling each cycle listed bellow.  \begin{itemize}
    \item $S_1 = \{(1,b,4,c),(1,c,4,d),(1,b,4,d)\}$ 
    \item $S_2 = \{(2,b,4,c),(2,c,4,d),(2,b,4,d)\}$ 
    \item $S_3 = \{(3,b,4,c),(3,c,4,d),(3,b,4,d)\}$
\end{itemize} 
 Notice that by B\"ohme's lemma we can simultaneously bound a disk in each of these cycles to make 3 spheres. Note that since 1,2 and 3 are all connected to $a$, the following is without loss of generality. Since 1 and 2 are  connected to $a$, by the Jordan-Brouwer theorem $a$ must be placed between $S_1$ and $S_2$ so that the edge between $a$ and 2 and the edge between $a$ and 1 both lie in only one sphere. However, 3 is also connected to $a$ so the edge between 3 and $a$ must be split into two spheres which contradicts flatness.  Therefore, we have a contradiction and $K_{4,4} - e$ is not flat. Hence since $K_{4,4} - e$ is not flat, it is not spherically flat.

\item $P_7$

\begin{center}
\includegraphics{fixed p7.jpg}
\end{center}

Denote the six vertices of $K_6$ by $\{a,b,c,1,2,3\}$, and suppose that a $\Delta -Y$ exchange took place between $1,2,$ and $3$. By way of contradiction, suppose that $P_7$ is flat. Consider the induced subgraphs formed by the sets of vertices below:\begin{itemize}
    \item $G_1 = G[\{a,b,c,1\}]$ 
    \item $G_2 = G[\{a,b,c,2\}]$ 
    \item $G_3 = G[\{a,b,c,3\}]$
\end{itemize}

B\"ohme spheres formed by the panellings $\mathcal{B}_1 = \{(1,a,2,v),(1,a,2,b),(1,v,2,b)\}, \mathcal{B}_2 = \{(1,a,2,v),(1,a,2,c),(1,v,2,c)\},$ and $\mathcal{B}_3= \{(1,a,2,v),(1,a,3,v),(2,a,3,v)\}$.
\begin{center}
\includegraphics{p7_pyramids.jpg}
\end{center}
As $b$ and $3$ are connected by an edge and $3$ is on the outside of the sphere formed by $\mathcal{B}_2$, $b$ is on the outside of the sphere formed by $\mathcal{B}_2$. But as $3$ is on the inside of the sphere formed by $\mathcal{B}_2$, $b$ is on the outside of the sphere formed by $\mathcal{B}_2$, which is a contradiction. Thus, $P_7$ is not flat.
\item $P_8$
\begin{center}
\includegraphics{p8withv2.png}
\end{center}

 By way of contradiction, suppose that $P_8$ is flat. Consider the induced subgraphs 
\begin{itemize}
    \item $G_1 = G[a,y,1,b,2,v]$
    \item $G_2 = G[a,y,1,b,2,c]$
    \item $G_3 = G[a,y,1,b,2,3]$
\end{itemize}
and their respective B\"ohme spheres formed by their panelling
\begin{itemize}
    \item $\mathcal{B}_1 = \{(a,y,1,b,2),(v,2,a,y),(v,y,1,b),(v,b,2)\}$
    \item $\mathcal{B}_2 = \{(a,y,1,b,2),(a,y,1,c,2),(b,1,c,2)\}$
    \item $\mathcal{B}_3 = \{(a,y,1,b,2),(a,y,1,b,3),(a,2,b,3)\}$
\end{itemize}
 Without loss of generality, as $v$ and $3$ are connected by an edge, by the Jordan-Brouwer Theorem, both $v$ and $3$ are on the outside of the sphere formed by $\mathcal{B}_2$. Then, either $v$ is inside of the sphere formed by $\mathcal{B}_3$ or $3$ is outside the sphere formed by $\mathcal{B}_1$. Without loss of generality, suppose $v$ is inside of $\mathcal{B}_3$. Then, as $v$ is connected to $c$ and $v$ is inside of $\mathcal{B}_1$, $c$ is inside of $\mathcal{B}_1$ by the Jordan-Brouwer Theorem. As $c$ is connected to $3$, 3 is inside of $\mathcal{B}_1$ by the Jordan-Brouwer Theorem. However, the edge connecting 3 and $v$ is both inside and outside of $\mathcal{B}_2$, which contradicts the Jordan-Brouwer Theorem. Thus, $P_8$ is not flat.



\item $P_9$

\begin{center}
    \includegraphics{p9.jpg}
\end{center}

Assume by way of contradiction that $P_9$ is flat. Then by definition of flat, there is a spacial embedding, such that for each cycle there is a disk bounded by the cycle with an interior disjoint from the rest of the graph. Consider the spheres ($S_i$ where $i \in \{1,2,3\}$) formed by panelling each cycle listed bellow.  \begin{itemize}
    \item $S_1 = \{(1,2,3,4,5,6),(6,7,3,4,5),(6,7,3,2,1)\}$ 
    \item $S_2 = \{(1,2,3,4,5,6),(2,8,5,4,3),(2,8,5,6,1)\}$ 
    \item $S_3 = \{(1,2,3,4,5,6),(1,9,4,3,2),(1,9,4,5,6)\}$
\end{itemize} 
 Notice that by B\"ohme's lemma we can simultaneously bound a disk in each of these cycles so each $S_i$ forms a sphere for $i=1,2,3$. Since 8 and 9 are connected, by the Jordan-Brouwer theorem, 8 and 9 are either both in the outside region or both in the inside region of $S_1$. Without loss of generality assume 8 and 9 are in the outside region of $S_1$. Note that since 8,9, and 7 are all connected the following is without loss of generality. Then since 8 is connected to 7, by the Jordan-Brouwer theorem, $S_1$ must lie in the inside region of $S_2$. Similarly since 8 is connected to 9, by the Jordan-Brouwer theorem, $S_2$ must lie in the inside region of $S_3$. However, 9 is connected to 7, and hence the edge connecting 9 and 7 is in both the outside and inside region of $S_2$ which is not possible according to the Jordan-Brouwer theorem. Thus we have a contradiction and therefore, $P_9$ is not flat.

%Let $x$ be the extra vertex formed as a result of a $Y-\Delta$ exchange between $a,1,$ and $v$ of $K_{3,3,1}$ and let $y$ be the extra vertex formed as a result of a $Y-\Delta$ exchange between $b,2,$ and $v$. By way of contradiction, suppose $P_9$ is flat. Consider the B\"ohme spheres formed by the panellings $\mathcal{B}_1 = \{(a,x,1,b,y,2),(a,x,1,c,2),(1,c,2,y,b)\},\mathcal{B}_2 = \{(a,x,1,b,y,2),\\(a,3,b,1,x),(a,3,b,y,2)\}$, and $\mathcal{B}_3 = \{(a,x,1,b,y,2),\\(a,x,v,y,2),(1,x,v,y,b)\}.$ By the Jordan-Brouwer Theorem, as $v$ and $c$ are connected by an edge and $v$ is on the outside of the sphere formed by $\mathcal{B}_2$, $c$ is on the outside of the sphere formed by $\mathcal{B}_2$. But as $c$ is on the inside of the sphere formed by $\mathcal{B}_2$, $v$ is on the inside of the sphere formed by $\mathcal{B}_2$. 



\item $P_{10}$

\begin{center}
    \includegraphics{P_10.jpg}
    \includegraphics{p10.jpg}
\end{center}


Suppose by way of contradiction that $P_{10}$ is flat. Then by definition of flat, there is a spacial embedding, such that for each cycle there is a disk bounded by the cycle with an interior disjoint from the rest of the graph. Consider the induced subgraphs formed by each set of vertices below.  \begin{itemize}
    \item $G_1 = G[\{1,2,3,4,5,6,9\}]$ 
    \item $G_2 = G[\{1,2,3,4,5,7,10\}]$ 
    \item $G_3 = G[\{1,2,3,4,5,6,8\}]$
\end{itemize} 
Then by B\"ohme's lemma we can simultaneously bound disks in each 5-cycle and 6-cycle in $G_1,G_2,$and $G_3$ to form 3 spheres. Note that the cycle $(1,2,3,4,5)$ is in each induced subgraph as each sphere shares the same bottom base.
    By Jordan Brouwer Theorem, since 7 is connected to 10, they must both be outside or both be inside of the sphere formed by $G_1$. Without loss of generality, assume they are both outside. Then the sphere created by $G_2$ lays in the closure of the region outside of the sphere created by $G_1$. Since 8 is connected to both 6 and 10, 8 must be between the sphere created by $G_2$ and the sphere created by $G_1$. Now the sphere formed by $G_3$ is sandwiched between the sphere created by $G_2$ and the sphere created by $G_1$. But now since 7 is connected to 9, and 7 is in $G_2$ and 9 is in $G_1$, the sphere formed by $G_3$ intersects the edge connecting 7 to 9. However, based on how these spheres were formed we cannot place 7 and 9 on the same side of sphere formed by $G_3$. So we are contradicting flattness since the sphere generated by $G_3$ was punctured, hence a paneled disk must have been punctured. Therefore, $P_{10}$ is not flat and thus not spherically flat.
\end{itemize}

\section{$\Delta - Y$ preserves spherically flat}
\textbf{Theorem:} $\Delta - Y$ preserves spherically flat.
First we will prove that Y-$\Delta$ preserves not spherically flat.

\textbf{Proof:} Suppose $G_Y$ is not spherically flat. Let $G_{\Delta}$ be obtained from $G_Y$ by a $Y-\Delta$ exchange. Let $f(G_{\Delta})$ be an arbitrary embedding of $G_{\Delta}$. If  $\Delta$ cannot be paneled, then $f(G_{\Delta})$ is not a flat embedding of $G_{\Delta}$ and thus is not a spherically flat embedding. Hence assume $\Delta$ can be paneled. Consider for all $G_y-\{Y\}$, $f'(G_y)=f(G_{\Delta})$ and for $Y$, lay $Y$ within the disk bounded by $\Delta$ where $Y$ connects to the vertices of $\Delta$. Since $G_Y$ is not spherically flat, and $f'(G_y)$ is a spatial embedding of $G_Y$, there exists planar subgraph $P_Y$ of $G_Y$ such that every sphere that contains $P_Y$ intersects $f'(G_Y)-f'(P_Y)$, and we can assume transversally and minimally. Since $P_Y$ is planar and because of the way $G_Y$ was embedded, there is a corresponding planar subgraph of $G_{\Delta}$,  $P_{\Delta}$. Let $S_{P_{\Delta}}$ be an arbitrary sphere containing $P_{\Delta}$. Then for the embedding of $G_Y$ there is a corresponding sphere containing $P_Y$, called $S_{P_Y}$. Notice that $S_{P_Y}$ intersects $f'(G_Y)-f'(P_Y)$.

Case 1: Suppose $f'(P_Y)$ is completely disjoint from $Y$ in $f'(G_Y)$. Then $Y$ is in $f'(G_Y)-f'(P_Y)$ and $\Delta$ is in $f(G_{\Delta})-f(P_{\Delta})$. Thus $S_{P_Y}$ could intersect $Y$ or not.

Subcase a: Suppose $S_{P_Y}$ intersects $Y$ transversally and minimally. Then $S_{P_Y}$ intersects some 2-path in $Y$ and since every 2-path is ambient isotopic to an edge of $\Delta$, $S_{P_{\Delta}}$ must intersect $\Delta$ transversally and minimally through the corresponding edge. Then $S_{P_{\Delta}}$ intersects $f(G_{\Delta})-f(P_{\Delta})$ as $\Delta$ is in $f(G_{\Delta})-f(P_{\Delta})$.

Subcase b: Suppose $S_{P_Y}$ does not intersect $Y$. Then $S_{P_Y}$ intersects some other subgraph of $f'(G_Y)-f'(P_Y)$. Since this subgraph is in $G_Y-Y$, $f'(G_Y)=f(G_{\Delta})$ for this subgraph. Thus since $S_{P_Y}$ intersects $f'(G_Y)-f'(P_Y)$ transversally and minimally, and since this intersection is unchanged by $Y-\Delta$, $S_{P_{\Delta}}$ intersects $f(G_{\Delta})-f(P_{\Delta})$ transversally and minimally. 

Thus in both cases, $S_{P_{\Delta}}$ intersects $f(G_{\Delta})-f(P_{\Delta})$.

Case 2: Suppose $P_Y$ contains just some vertices or edges of $Y$ but not all. Then there is a piece of $Y$ which is in $f'(G_Y)-f'(P_Y)$ and a piece of $\Delta$ is in $f(G_{\Delta})-f(P_{\Delta})$. Then we have the same subcases from case one, but with just a piece of $Y$ and a piece of $\Delta$. However, the reasoning of these two subcases remains the same regardless of just having a piece of $Y$ and $\Delta$. Hence we can conclude that $S_{P_{\Delta}}$ intersects $f(G_{\Delta})-f(P_{\Delta})$.


Case 3: Suppose $Y$ is a subgraph of $P_Y$. Then $S_{P_Y}$ intersects $f'(G_Y)-f'(P_Y)$ at a point not in $Y$. Hence, from Case 1 Subcase b, $S_{P_{\Delta}}$ intersects $f(G_{\Delta})-f(P_{\Delta})$.

Hence in every possible case, $S_{P_{\Delta}}$ intersects $f(G_{\Delta})-f(P_{\Delta})$. So for all $f(G_{\Delta})$ there exists a planar subgraph $P_{\Delta}$ such that every sphere containing $P_{\Delta}$ intersects $f(G_{\Delta})-f(P_{\Delta})$. Therefore, $G_{\Delta}$ is not spherically flat.

\bigskip 
Now we have shown that Y-$\Delta$ preserves not spherically flat. So by contrapositive we have that $\Delta$-Y preserves spherical flatness.
 


 

\begin{thebibliography}{9}

\bibitem{adams} Adams, C., The Knot Book, AMS, 2004.

 

\bibitem{bohme}

B\"ohme, T., On spatial representations of graphs, Contemporary Methods in Graph Theory (R. Bodendieck, Ed.), Mannheim, Wien, Zurich, 1990, pp. 151-167.

 

\bibitem{cg} Conway, J. and Gordon, C.  \textit{Knots and links in spatial graphs}. J. Graph Theory 7 (1983), no. 4, 445-453.


\bibitem{df} Dehkordi, H., Farr, G.; Non-separating planar graphs, . Electron. J. Combin. 28 (2021), no. 1, Paper No. 1.11, 20 pp.

 

\bibitem{kur}

Kuratowski, Kazimir, \textit{Sur le probleme des courbes gauches en topologie}, Fund. Math. 15 (1930), 271-283.

           

\bibitem{robertson seymour thomas}

            Robertson, Seymour, and Thomas.  \textit{Linkless Embeddings of Graphs in 3-Space}.  Bulletin (New Series) of the American Mathematical Society.  Vol 28, No. 1. Jan 1993.

           

\bibitem{sachs}

            Sachs, H. \textit{On spatial representations of finite graphs}. Finite and infinite sets, Vol. I, II (Eger, 1981), 649‚Ai662, Colloq. Math. Soc. Janos Bolyai, 37, North-Holland, Amsterdam, 1984.

           

\bibitem{west}

West, Stephen, Introduction to Graph Theory, Prentice Hall, Inc., Upper Saddle River, NJ, 1996.

 

%\bibitem{whit}

%Whitney, H., 2-isomorphic graphs, Amer. J. Math 55 (1933), 245-254.

%\bibitem{wu}

            %Wu, Ying-Quing.  \textit{On planarity of graphs in 3-manifolds}.  Commentarii Mathematici Helvetici.  67(1992), no. 4, 635-647. 

           

           

           

           

 

\end{thebibliography}
\end{document}

